Deterministic Decremental Reachability, SCC, and Shortest Paths via Directed Expanders and Congestion Balancing

Let $G = (V,E,w)$ be a weighted, digraph subject to a sequence of adversarial edge deletions. In the decremental single-source reachability problem (SSR), we are given a fixed source $s$ and the goal is to maintain a data structure that can answer path-queries $s \rightarrowtail v$ for any $v \in V$. In the more general single-source shortest paths (SSSP) problem the goal is to return an approximate shortest path to $v$, and in the SCC problem the goal is to maintain strongly connected components of $G$ and to answer path queries within each component. All of these problems have been very actively studied over the past two decades, but all the fast algorithms are randomized and, more significantly, they can only answer path queries if they assume a weaker model: they assume an oblivious adversary which is not adaptive and must fix the update sequence in advance. This assumption significantly limits the use of these data structures, most notably preventing them from being used as subroutines in static algorithms. All the above problems are notoriously difficult in the adaptive setting. In fact, the state-of-the-art is still the Even and Shiloach tree, which dates back all the way to 1981 and achieves total update time $O(mn)$. We present the first algorithms to break through this barrier: 1) deterministic decremental SSR/SCC with total update time $mn^{2/3 + o(1)}$ 2) deterministic decremental SSSP with total update time $n^{2+2/3+o(1)}$. To achieve these results, we develop two general techniques of broader interest for working with dynamic graphs: 1) a generalization of expander-based tools to dynamic directed graphs, and 2) a technique that we call congestion balancing and which provides a new method for maintaining flow under adversarial deletions. Using the second technique, we provide the first near-optimal algorithm for decremental bipartite matching.

==> components_backup.tex <==

\section{The Main Components}

\label{sec:ingredient}

\subsection{Witness Maintenance}

\begin{defn}
[Witness]\label{def:witness}We say that $W$ is a\emph{ $\phi$-witness}
of $G$ if $V(W)\subseteq V(G)$, $W$ is a $1/n^{o(1)}$-expander,
and there is an embedding $\pset$ with vertex-congestion $1/\phi$
We say that $W$ is a $\phi$-{\emph short}-witness if it is a $\phi$-witness and the embedding has length $\Ohat(1/\phi)$. We say that $W$ is a \emph{large} witness if $|V(W)|\ge|V(G)|/2$.
\end{defn}

Note that $E(W)$ might not be a subset of $E(G)$.

We will also define the edge congestion version of witness in \ref{def:witness edge}.
But we do not need it here.
\begin{rem}
If $W$ has high sparsity, then $G$ will not have balanced sparse
cut. But here, $W$ has only high conductance, $G$ may have balanced
sparse cut. But this is not a problem for us. Also, it is easy to make
$W$ has high sparsity.
\end{rem}

\begin{thm}
[Robust Witness Maintenance]\label{thm:robust witness}There is a
deterministic algorithm that $\rwitness(G,\phi)$ that takes as input  a directed decremental $n$-vertex
graph $G$ and a parameter $\phi \in (0,1\log^2(n)]$. The algorithm maintains a large (weighted) $\phi$-witness $W$ of $G$ using $\Ohat(m/\phi^{2})$
total update time such that every edge weight in $W$ is a positive multiple of $1/d$, for some $d \leq 2\davg$, where $\davg$ is an initial average degree of $G$. The total edge weight in $W$ is $O(n\log n)$. At every stage,
the algorithm either updates $W$ or outputs a $(\phi n^{o(1)})$-vertex-sparse
$(1/n^{o(1)})$-vertex-balanced vertex-cut and terminates. 

Let $W^{(i)}$ be $W$ after the $i$-th update. There exists a set
$R$ of \emph{reset indices} where $|R|=\Ohat(\phi^{-1})$ such that,
for each $i\notin R$, $W^{(i)}\supseteq W^{(i+1)}$. That is, the
algorithm has $\Ohat(\phi^{-1})$ phases such that, within each phase,
$W$ is a decremental graph. The algorithm also reports at the beginning
of each phase. 

The algorithm also explicitly maintains the embedding $\pset$ that
embeds $W$ into $G$.
\end{thm}

\begin{example}
[Bad Witness Maintenance]{[}TODO add to overview?{]}. If we start
from a complete graph $G$ and $W$ is unweighted. We might need to
embed $W$ $n$ times. Our robust witness maintenance only need to
embed $W$ $n^{o(1)}$ times. 
\end{example}


\subsection{Shallow Forest Rooted at Witness}

An \emph{out-tree} is a rooted tree where all edges directed outward
from the root. An \emph{out-forest} is a collection of out-trees.
In-trees and in-forests are defined similarly.

\textbf{Note: }When we use \ref{thm:ES from witness} to prove the
main result in \ref{sec:SCC}, $W$ will be maintained as a decremental
large $\phi$-witness.

\textbf{TODO: }define: forest rooted at $W$ and $\dist_{F_{in}}(a,V(W))$. 
\begin{thm}
\label{thm:ES from witness}There is a deterministic algorithm that,
given a parameter $\phi>0$, a directed $m$-edge decremental graph
$G$, and a decremental graph $W$ where $V(W)\subseteq V(G)$, in
$\tilde{O}(m\phi^{-1})$ total update time, maintains a decremental
set $A$ such that $A=V(G)$ initially, and $A\supseteq V(W)$ at
any time, and whenever the set $A$ is updated to $A'$, the algorithm
outputs a $\phi$-vertex-sparse vertex cut $(L,S,R)$ of $G[A]$ where
$|L|\le|R|$ and $R=A'$.

Additionally, as long as $W\neq\emptyset$, the algorithm explicitly
maintains directed out-forest $F_{out}$ and in-forest $F_{in}$ rooted
at vertices in $W$ such that, for all $a\in A$, $\dist_{F_{in}}(a,V(W))=O(\phi^{-1}\log m)$
and $\dist_{F_{out}}(V(W),a)=O(\phi^{-1}\log m)$. 
\end{thm}


\subsection{Short Path Oracles on Witness}
\begin{thm}
\label{thm:short-path-oracle}There is a deterministic algorithm,
that given a directed $n$-vertex $m$-edge graph $W=(V,E)$ with
undergoing edge deletions and vertex deletions with a promise that
$W$ is a $\phi$-expander at any stage where $\phi=1/n^{o(1)}$,
in $\Ohat(m)$ total update time, maintains a data structure that
given any pair of vertices $u,v\in V(W)$, return a directed simple
path $P_{uv}$ from $u$ to $v$ and a directed simple path $P_{vu}$
of $v$ to $u$ both of length at most $n^{o(1)}$ in $n^{o(1)}$
time.
\end{thm}


\subsection{Lacki's Scheme}
\begin{prop}
\label{thm:Lacki}Suppose there is a data structure that, given a
decremental $m$-edge $n$-vertex graph $G=(V,E)$, in total update
time $T(m,n)$,
\begin{enumerate}
\item maintains an incremental set $S\subset V$ 
\item maintains SCCs of $G-S$ explicitly , and
\item supports SCC queries in $G-S$ (in almost-path-length query time), 
\end{enumerate}
then there is a data structure that takes total update time $O(T(m,n)+m|S|)$
to
\begin{itemize}
\item maintain SCCs of $G$ explicitly, and
\item support SCC queries in $G$ (in almost-path-length query time).
\end{itemize}
\end{prop}


\subsection{Reduction for SSSP}

TODO: State blackbox for SSSP as well to avoid notation conflict.


==> flow.tex <==

\section{Implementation of Flow Subroutines}

\label{sec:flow}

Throughout this paper, we use several flow subroutines for various
contexts (e.g.~expander pruning, embedding robust witness, finding
approximate matching, etc.). All these flow algorithms are based on
the same techniques which is the \emph{bounded height variant} of
push-relabel and blocking flow algorithms. This idea was used explicitly
many times before (e.g.~\cite{LangR04,OrecchiaZ14,HenzingerRW17,SaranurakW19}).
Our contribution in this section is only to show a uniform presentation
that all of our flow subroutines can be implemented using the same
framework, and to give proofs for completeness.

We start with introducing notations in \Cref{sec:flow notation},
then we describe the guarantee of the bounded height variant of push-relabel
and blocking flow algorithms in \Cref{sec:bounded height flow}.
All the flow subroutines share the same framework which is described
in \Cref{sec:flow framework}. Using this framework, we instantiate
the flow subroutines that we need throughout the paper in \Cref{sec:flow
subroutine}.

\subsection{Flow Notations}

\label{sec:flow notation}

The notation below is slight adjusted from \cite{SaranurakW19} because
we work with directed graphs instead of undirected graphs.

A \emph{flow problem} $\Pi$ on a \emph{directed} graph $G=(V,E)$
is specified by a source function $\Delta:V\rightarrow\mathbb{R}_{\geq0}$,
a sink capacity function $T:V\rightarrow\mathbb{R}_{\geq0}$, and
edge capacities $c:E\rightarrow\mathbb{R}_{\geq0}$. We say that $\Pi$
is \emph{integral} if $\Delta:V\rightarrow\mathbb{Z}_{\geq0}$, $T:V\rightarrow\mathbb{Z}_{\geq0}$,
and $c:E\rightarrow\mathbb{Z}_{\geq0}$. More generally, for any number
$d\ge1$, we say that $\Pi$ is $1/d$-integral if $\Delta:V\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$,
$T:V\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$, and $c:E\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$.
We use \emph{mass} to refer to the substance being routed. For a vertex
$v$, $\Delta(v)$ specifies the amount of mass initially placed on
$v$, and $T(v)$ specifies the capacity of $v$ as a sink. For an
edge $e$, $c(e)$ bounds how much mass can be routed along the edge.

A \emph{routing} (or \emph{flow}) $f:E\rightarrow\mathbb{R}_{\ge0}$
is $1/d$-integral if $f:E\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$.
$f(u,v)>0$ means that mass is routed in the direction from $u$ to
$v$. If $f(u,v)=c(u,v)$, then we say $(u,v)$ is \emph{saturated}.
Given $\Delta$, we also treat $f$ as a function on vertices, where
$f(v)=\Delta(v)+\sum_{u}f(u,v)$ is the amount of mass ending at $v$
after the routing $f$. If $f(v)\ge T(v)$, then we say $v$'s sink
is \emph{saturated}. For $A,B\subset V$, let $f(A,B)=\sum_{(u,v)\in E\cap(A\times B)}f(u,v)$
be the total mass routing directly from $A$ to $B$.

We say that $f$ is a \emph{feasible routing/flow} for $\Pi$ if $f(u,v)\leq c(u,v)$
for each edge $e=(u,v)$ (i.e.~obey edge capacities), $\sum_{u}f(v,u)\leq\Delta(v)$
for each $v$ (i.e.~the net amount of mass routed away from a vertex
can be at most the amount of its initial mass), and $f(v)\leq T(v)$
for each $v$ (i.e.~no excess flow on each vertex).

Given a flow problem $\Pi=(\Delta,T,c)$, a \emph{pre-flow} $f$ is
a feasible routing for $\Pi$ except the condition $\forall v:f(v)\leq T(v)$
may not be satisfied. As pre-flow may not obey sink capacity on vertices,
we define the \emph{absorbed} mass on a vertex $v$ as $\ab_{f}(v)=\min(f(v),T(v))$.
We have $\ab_{f}(v)=T(v)$ iff $v$'s sink is saturated. The \emph{excess}
on $v$ is $\ex_{f}(v)=f(v)-\ab_{f}(v)$. From the definition, when
there is no excess, $\forall v:\ex_{f}(v)=0$, then $f$ is a feasible
flow for $\Pi$. Intuitively, we think of $\max\{\Delta(v)-T(v),0\}$
as \emph{initial excess} at $v$, and $\ex_{f}(v)$ is the excess
at $v$ after routing $f$. Similarly, we think of $\min\{\Delta(v),T(v)\}$
as \emph{initial absorbed mass} at $v$ and $\ab_{f}(v)$ is the absorbed
mass at $v$ after routing $f$. For any $S\subseteq V$, we usually
write $x(S)=\sum_{v\in S}x(v)$ where $x$ can be from $\{\Delta,T,\ex_{f},\ab_{f}\}$
(e.g.~$\Delta(S)$, $\ab_{f}(S)$). We omit the subscript whenever
it is clear.

For any directed path $P$, let $|P|$ denote the number of edges
in $P$. A \emph{path-decomposition} of a pre-flow $f$ is a collection
$\pset_{f}$ of directed paths with \emph{value} $\val(P)>0$ associated
with each path $P\in\pset_{f}$ and $\sum_{P\in\pset_{f}\mid P\ni e}\val(P)=f(e)$
for all $e\in E$.

\subsection{Bounded Height Push-Relabel and Blocking Flow}

\label{sec:bounded height flow}

The following proposition is the key algorithmic component for the
whole section. 
\begin{prop}
\label{prop: preflow and label}There is an algorithm that, given
a directed $n$-vertex $m$-edge graph $G=(V,E)$, a height parameter
$h\ge1$, and a flow problem $\Pi=(\Delta,T,c)$, returns a preflow
$f$ together with labels on vertices $l:V\rightarrow\{0,\dots,h\}$
such that: 
\begin{enumerate}
\item \label{enu:cross for}If $l(u)>l(v)+1$ and $(u,v)\in E$, then the
mass on $(u,v)$ is saturated, i.e.,~$f(u,v)=c(u,v)$. 
\item \label{enu:cross back}If $l(u)>l(v)+1$ and $(v,u)\in E$, then the
mass on $(v,u)$ is empty, i.e.,~$f(v,u)=0$. 
\item \label{enu:no excess}If $l(v)<h$, then $v$ has no excess, i.e.~$\ex_{f}(v)=0$. 
\item \label{enu:full absorb}If $l(v)>0$, then $v$'s sink is saturated,
i.e.~$\ab_{f}(v)=T(v)$. 
\item \label{enu:monotone}After routing $f$, excess does not increase
and absorbed mass never decreases, i.e.~$\ex_{f}(v)\le\max\{\Delta(v)-T(v),0\}$
and $\ab_{f}(v)\ge\min\{\Delta(v),T(v)\}$ for all $v$. 
\end{enumerate}
The algorithm takes at most $O(mh\log m)$ time. If $\Pi$ is $1/d$-integral
for some number $d\ge1$, then so is $f$. If $\Pi$ is integral,
$T(v)\ge\deg(v)$ for all $v\in V$, and the algorithm can access
the adjacency list of every vertex, then the running time can be reduced
to $O(\Delta(V)h)$. 

\end{prop}

\begin{proof}
The statement simply summarizes the output that one can obtain from
performing blocking flow computations for $\approx h$ rounds (instead
of $\approx n$ rounds as when we want to solve the exact max flow
problem).

We explain this idea in more detail. Let us create a graph $G'$ from
the graph $G$ by adding a super source vertex $s$ and a super sink
vertex $t$. For each $u\in V$, we add an edge $(s,u)$ with capacity
$\Delta(u)$. For each $u\in V$, we add an edge $(u,t)$ with capacity
$T(u)$. Then, we run blocking flow for at most $h+2$ rounds until
the (unweighted) distance between $s$ and $t$ in the residual graph
$G'_{f}$ of $G'$ is at least $h+2$. Each blocking flow computation
takes $O(m\log m)$ time (even when the flow problem $\Pi$ is fractional).
This running time is possible by using the \emph{link-cut tree data
structure}. (See the detail in Section 6 of \cite{SleatorT83}, Page
387-389.) So the total running time is $O(mh\log m)$. This completes
the running time analysis.

Let $f$ be the flow in $G'$ obtained after the blocking flow computations.
We can define the vertex labeling $l:V\cup\{s,t\}\rightarrow\{0,\dots,h\}$
as follows. For $0\le i\le h$, we set $l(u)=h-i+1$ where $i$ is
the (unweighted) distance between $s$ and $u$ in $G'_{f}$. For
all vertices $u$ whose distance from $s$ is more than $h$, we set
$l(u)=0$. By definition, $l(s)=h+1$. Also, as the distance from
$s$ to $t$ in $G'_{f}$ is $h+2$, for each label $i\in\{0,\dots,h\}$,
there must exist a vertex with label $i$. Observe that, for any edge
$(u,v)$ where $|l(u)-l(v)|>1$, the residual capacity in $G'_{f}$
must be $c_{f}(u,v)=0$. So this implies \Cref{enu:cross for} and
\Cref{enu:cross back}.

Note that we can view $f$ as a preflow on $G$ by restricting $f$
to only edges of $G$. Observe that the flow value on $(u,t)$ in
$G'$ corresponds to the absorbed flow at $u$ in $G$, i.e.~$f(u,t)=\ab_{f}(u)$.
Also, the residual capacity $c_{f}(s,u)$ of $(s,u)$ in $G'_{f}$
corresponds to the excess at $u$ after routing $f$, i.e.~$c_{f}(s,u)=\Delta(u)-f(s,u)=\ex_{f}(u)$.
So if $l(u)<h$, then $c_{f}(s,u)=0$ and so $\ex_{f}(u)=0$. Also,
if $l(u)>0$, then $c_{f}(u,t)=0$ and so $\ab_{f}(u)=T(u)$. This
implies \Cref{enu:no excess} and \Cref{enu:full absorb}.

In fact, our algorithm will do some simple preprocessing. For each
$u$, we will assume that we start with the initial flow that go through
$(s,u)$ and $(u,t)$ with value $\min\{\Delta(u),T(u)\}$. So initially
there are $\min\{\Delta(u),T(u)\}$ units of mass absorbed at $u$
and the initial excess at $u$ is $\max\{\Delta(u)-T(u),0\}$. As
the blocking flow computations have a property that flow value incident
to $s$ and $t$ never decreases. This implies \Cref{enu:monotone}.
This completes the correctness of the algorithm with running time
$O(mh\log m)$. Note that the implementation of blocking flow using
link-cut tree also have the guarantee that flow value on each edge
is $1/d$-integral if the given flow problem $\Pi$ is $1/d$-integral.

Lastly, we need to show if $\Pi$ is integral, $T(v)\ge\deg(v)$ for
all $v\in V$, and the algorithm can access the adjacency list of
every vertex, then the running time is $O(\Delta(V)h)$. However,
the proposition here is simply the summary of the output by the Unit
Flow algorithm by Henzinger Rao and Wang \cite{HenzingerRW17} (see
also \cite{SaranurakW19}) where Unit Flow is a bounded height variant
of push-relabel algorithms. 
\end{proof}
\begin{lem}
\label{lem:path decomposition}Given a preflow $f$ from the algorithm
from \Cref{prop: preflow and label}, any path decomposition $\pset_{f}$
of $f$ satisfies $\sum_{P\in\pset_{f}}\val(P)|P|\le\Delta(V)h$.
Moreover, if the flow problem $\Pi$ is $1/d$-integral, then a decomposition
$\pset_{f}$ can be computed in time $O(\sum_{P\in\pset_{f}}|P|)=O(d\Delta(V)h)$. 
\end{lem}

\begin{proof}
By the definition of path decomposition, we have $\sum_{P\in\pset_{f}\mid P\ni e}\val(P)=f(e)$
for all $e\in E$. So 
\[
\sum_{P\in\pset_{f}}\val(P)|P|=\sum_{e\in E}\sum_{P\in\pset_{f}\mid P\ni e}\val(P)=\sum_{e\in E}f(e).
\]
Now, we want to show that $\sum_{e\in E}f(e)\le\Delta(V)h$. Consider
the bounded height blocking-flow algorithm or push-relabel algorithm.
The algorithm always sends the flow along a path of length at most
$h$ in the residual graph. So even the total flow value over all
edges ``without flow cancellation'' must be at most $\Delta(V)h$.
As $\sum_{e\in E}f(e)$ is the total flow value over all edges ``after
flow cancellation'', we conclude that $\sum_{e\in E}f(e)\le\Delta(V)h$.

We can find a path decomposition $\pset_{f}$ of a flow $f$ in time
$O(\sum_{P\in\pset_{f}}|P|)$ as follows. As the flow problem $\Pi$
is $1/d$-integral, the flow value of each edge $f(e)$ is also $1/d$-integral
by \Cref{prop: preflow and label}. Let $H$ be a graph induced
by edges $e$ where positive flow value $f(e)>0$. We make $H$ unweighted
by scaling up all edges in $H$ by a factor of $d$. Then, we add
a dummy source to $H$ and performing the depth-first search on $H$
from the dummy source. Whenever a search reaches a sink $u$ (i.e.
$\ab_{f}(u)>0$) or the search cannot proceed from $u$ (i.e. $\ex_{f}(u)>0$),
we backtrack and output the corresponding path $P$ excluding the
dummy source. Note that $P$ is a directed \emph{simple} path in $H$
and corresponds to a flow path of value $1/d$. We remove the path
$P$ from $H$ and repeat.

Observe that each edge in $H$ is read at most twice and so the total
time is subsumed by the total time for outputting all paths which
is $O(\sum_{P\in\pset_{f}}|P|)$. As $\val(P)\ge1/d$, so $O(\sum_{P\in\pset_{f}}|P|)\le O(\sum_{P\in\pset_{f}}d\cdot\val(P)|P|)=O(d\Delta(V)h)$. 
\end{proof}
For convenience, we will use the following notation throughout this
section. 
\begin{defn}
Given a vertex labeling $l:V\rightarrow\{0,\dots,h\}$, let $V_{i}=\{u\mid l(u)=i\}$
for each $i$. Also, we define $V_{\ge i}=\{u\mid l(u)\ge i\}$ and
$V_{>i},V_{\le i},V_{<i}$ are defined similarly. 
\end{defn}

When the input graph to \Cref{prop: preflow and label} is bipartite
and all source/sink vertices are only on the left/right respectively,
we can additionally guarantee that the vertices from each level alternate
between the left and right side of the bipartite graph $G$. 
\begin{lem}
\label{lem:bipartite label}If the input graph from \Cref{prop:
preflow and label} is a bipartite graph $G=(L,R,E)$ where $R$ has
no initial mass ($\Delta(R)=0$), and $L$ cannot absorb mass ($T(L)=0$),
then the vertex labeling $l$ from \Cref{prop: preflow and label}
has additional property that $V_{h},V_{h-2},V_{h-4},\dots\subseteq L$
and $V_{h-1},V_{h-3},V_{h-5},\dots\subseteq R$. 
\end{lem}

\begin{proof}
This guarantee follows immediately when we use blocking-flow-based
algorithms. For Unit Flow (push-relabel-based algorithm), we can guarantee
this using very simple modification: we initialize by assigning all
all vertices in $L$ a label $1$ and all vertices in $R$ a label
$0$, and when ever we relabel a vertex $l(u)\gets l(u)+1$, we instead
set $l(u)\gets l(u)+2$. All the invariants of the push-relabel-based
algorithm will still be maintained because the graph is bipartite. 
\end{proof}

\subsection{The Common Framework}

\label{sec:flow framework}

Given a flow problem $\Pi=(\Delta,T,c)$ for a graph $G=(V,E)$, all
the algorithms in \Cref{sec:flow subroutine} starts by calling
\Cref{prop: preflow and label} with parameter $h$ and obtain a
preflow $f$ and a vertex labeling $l:V\rightarrow\{0,\dots h\}$.

If the total excess after routing $f$ is at most $z$, then the algorithm
just returns $f$ and we are done. Otherwise, the algorithm will return
one of the \emph{level-$i$ cuts} $(V_{\ge i},V_{<i})$ for some $0<i\le h$.
The only main task we need to prove in each algorithm is to show that
there exists an index $i$ such that the level-$i$ cut satisfies
the requirement of the lemma.

There are two common arguments that will be used by all flow algorithms
in \Cref{sec:flow subroutine}. The first one will be used to lower
bound the ``size'' of both $V_{h}$ and $V_{0}$ by the total excess.
In our algorithm, the outputted cut $S$ will be such that $S\supset V_{h}$
and $S\cap V_{0}=\emptyset$, so the proposition below will be useful
to prove the balance of $(S,V\setminus S)$. 
\begin{prop}
\label{prop:excess give lower bound}If $\Delta(V)\le T(V)$, then
$\Delta(V_{h})\ge\ex_{f}(V)$ and $T(V_{0})\ge\ex_{f}(V)$.
\end{prop}

\begin{proof}
First, note that $\ex_{f}(V)=\ex_{f}(V_{h})$ because all vertices
with level below $h$ has no excess by \Cref{enu:no excess} of
\Cref{prop: preflow and label}. Also, $\ex_{f}(V_{h})\le\Delta(V_{h})-T(V_{h})$
because excess does not increase (\Cref{enu:monotone} of \Cref{prop:
preflow and label}). So $\ex_{f}(V)\le\Delta(V_{h})$. Similarly,
note that $T(V_{0})-\ab_{f}(V_{0})=T(V)-\ab_{f}(V)$ because all vertices
with level above $0$ are fully absorbed by \Cref{enu:full absorb}
of \Cref{prop: preflow and label}. Also, we have $T(V)-\ab_{f}(V)\ge\Delta(V)-\ab_{f}(V)=\ex_{f}(V)$
by the assumption that $T(V)\ge\Delta(V)$ and by the definition of
$\ex_{f}(V)$. So $\ex_{f}(V)\le T(V_{0})$. 
\end{proof}
The next common argument is for upper bounding the total capacity
of the level cut $(V_{\ge i},V_{<i})$. The argument used for bounding
capacity of ``consecutive-level'' edges from $E(V_{i},V_{i-1})$
will be different in each algorithm. But, the argument for bounding
total capacity of edges that are not from $E(V_{i},V_{i-1})$ will
be the same and is stated as follow: 
\begin{prop}
\label{prop:cap of skip}$c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))\le\Delta(V_{\ge i})+f(V_{i-i},V_{i})-\ab_{f}(V_{\ge i})-\ex_{f}(V_{\ge i})$. 
\end{prop}

\begin{proof}
First, note that each $(u,v)\in E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1})$
is ``skipping levels'', i.e.~$l(u)-l(v)>1$. So, by \Cref{enu:cross
for} of \Cref{prop: preflow and label}, we have $f(u,v)=c(u,v)$.
So the total capacity $c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))$
is at most the total mass going out of $V_{\ge i}$. Observe that
the total mass in-coming into $V_{\ge i}$ is $f(V_{i-i},V_{i})$
because any other edges $(u,v)\in E(V_{<i},V_{\ge i})\setminus E(V_{i-i},V_{i})$
is ``skipping levels'' and so $f(u,v)=0$ by \Cref{enu:cross back}
of \Cref{prop: preflow and label}. Therefore, the total mass going
out of $V_{\ge i}$ is at most 
\begin{align*}
\underset{\textrm{initial mass}}{\underbrace{\Delta(V_{\ge i})}}+\underset{\textrm{incoming mass}}{\underbrace{f(V_{i-i},V_{i})}}-\underset{\textrm{absorbed mass}}{\underbrace{\ab_{f}(V_{\ge i})}}-\underset{\textrm{excess}}{\underbrace{\ex_{f}(V_{\ge i})}}
\end{align*}
\end{proof}

\subsection{Flow Subroutines}

\label{sec:flow subroutine}

In this section, we state the flow subroutines that will be used by
several places throughout our paper. To state some lemmas below, we
also define degree and volume w.r.t. capacity function $c$. Given
a graph $G=(V,E)$ with edge capacity $c$, for $u\in V$, let $\deg^{c}(u)=\sum_{(u,v)}c(u,v)+\sum_{(v,u)}c(v,u)$
denote the weighted degree w.r.t.~$c$. For $S\subset V$, let $\vol^{c}(S)=\sum_{u\in S}\deg^{c}(u)$
be the volume of $S$ w.r.t.~$c$.

The following remark will be used repeatedly. 
\begin{rem}
\label{rem:excess at source and path decomposition} Let $f$ be a
preflow returned by any of the algorithms below in this section. Note
that every algorithm below starts by calling the algorithm from \Cref{prop:
preflow and label} with parameter $h$ on some graph. Note that any
vertex $v$ with positive excess, i.e.~$\ex_{f}(v)>0$, must have
positive initial excess, i.e.~$\Delta(v)-T(v)>0$. This follows from
\Cref{enu:monotone} of \Cref{prop: preflow and label}. By simply
scanning vertices with initial excess and removing excess after routing
$f$, we obtain a \emph{feasible flow} $f'$ of value $\Delta(V)-\ex_{f}(V)$
from $f$. The time to remove these excess is obviously subsumed by
the algorithm because the algorithm at least need to read all vertices
with initial excess. Moreover, we can obtain a path decomposition
of $f$ in additional time $O(d\Delta(V)h)$ if the flow problem is
$1/d$-integral by \Cref{lem:path decomposition}. 
\end{rem}


\subsubsection{Local Flow}

The algorithm below either sends most of the flow or finds a balanced
sparse cut in \emph{local} time. We need that the given flow problem
is integral and each vertex can absorb mass at least by its degree. 
\begin{lem}
[Local Flow]\label{lem:local flow}There is a deterministic algorithm
that, given access to the adjacency list of every vertex of a directed
$m$-edge graph $G=(V,E)$, parameters $z\ge0$ and $h\ge1$, and
an \emph{integral} flow problem $\Pi=(\Delta,T,c)$ with total capacity
$C=\sum_{e\in E}c(e)$ where 
\begin{enumerate}
\item $\forall v,\Delta(v)\le\overline{\Delta}\deg(v)$ and $T(v)\ge\deg(v)$
where $\deg(v)$ denote an unweighted degree of $v$ in $G$. 
\end{enumerate}
in $O(\Delta(V)\cdot h)$ time either 
\begin{itemize}
\item returns a preflow $f$ with total excess $\ex_{f}(V)\le z$, or 
\item returns a set $S$ where $z/\overline{\Delta}<\vol(S)\le\Delta(V)$
and $c(E(S,V\setminus S))\le\Delta(S)-T(S)-z+\vol^{c}(S)\cdot\frac{10\log C}{h}$. 
\end{itemize}
\end{lem}

\begin{proof}
We call \Cref{prop: preflow and label} with parameter $h$. By
the assumption of the lemma, the running time is $O(\Delta(V)h)$.
Suppose that $\ex_{f}(V)>z$ otherwise we are done. By \Cref{prop:excess
give lower bound}, we know $\vol(V_{h})\overline{\Delta}\ge\Delta(V_{h})>z$
because $\forall v\in V,\Delta(v)\le\overline{\Delta}\deg(v)$. So
$\vol(V_{h})>z/\overline{\Delta}$. Also, observe that $\vol(V_{\ge1})\le\Delta(V)$.
This is because all vertices in $V_{\ge1}$ are fully absorbed by
\Cref{enu:full absorb} of \Cref{prop: preflow and label}, so
$T(V_{\ge1})\le\ab_{f}(V_{\ge1})\le\Delta(V)$, and because $T(V_{\ge1})\ge\vol(V_{\ge1})$
as $T(v)\ge\deg(v)$ for all $v$.

By the ball growing argument, there is an index $0<i\le h$ such that
$c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i}))\le\min\{\vol^{c}(V_{\ge i}),\vol^{c}(V_{<i})\}\cdot\frac{10\log C}{h}$.
Otherwise, $\vol^{c}(V_{\ge1})\ge(1+\frac{10\log C}{h})^{h}>2C$ which
is a contradiction. We fix such $i$. Set $S=V_{\ge i}$. As $0<i\le h$,
so we have $z/\overline{\Delta}<\vol(S)\le\Delta(V)$. We have, by
\Cref{prop:cap of skip}, that 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{i},V_{i-1}))+c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))\\
 & \le c(E(V_{i},V_{i-1}))+\Delta(V_{\ge i})+f(V_{i-i},V_{i})-\ab_{f}(V_{\ge i})-\ex_{f}(V_{\ge i})\\
 & <\Delta(S)-T(S)-z+c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i})).
\end{align*}
By the choice of $i$, we are done. 
\end{proof}

\subsubsection{Global Flow}

The algorithm below either sends most of the flow or finds a balanced
sparse cut when the flow problem is fractional. This is needed because
the capacity of edges will be fractional when we maintain the robust
witness. 
\begin{lem}
[Global Flow]\label{lem:global flow}There is a deterministic algorithm
that, given a directed $m$-edge graph $G=(V,E)$, excess parameter
$z\ge0$, a height parameter $h\ge1$, and a flow problem $\Pi=(\Delta,T,c)$
with total capacity $C=\sum_{e\in E}c(e)$ where 
\begin{enumerate}
\item $\Delta(V)\le T(V)$, 
\item $\forall v\in V,\Delta(v),T(v)\le1$, 
\end{enumerate}
in $O(mh\log m)$ time, either 
\begin{itemize}
\item returns a preflow $f$ with total excess $\ex_{f}(V)\le z$, or 
\item returns a set $S\subset V$ where $|S|,|V\setminus S|>z$ and $c(E(S,V\setminus S))\le\Delta(S)-T(S)-z+\min\{\vol^{c}(S),\vol^{c}(V\setminus S)\}\cdot\frac{10\log C}{h}$. 
\end{itemize}
\end{lem}

\begin{proof}
We call \Cref{prop: preflow and label} with parameter $h$ in $O(mh\log m)$.
Suppose that $\ex_{f}(V)>z$. By \Cref{prop:excess give lower bound},
we know $|V_{h}|\ge\Delta(V_{h})>z$ and $|V_{0}|\ge T(V_{0})>z$
because $\forall v\in V,\Delta(v),T(v)\le1$. By the ball growing
argument applying in two directions, there is an index $0<i\le h$
such that $c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i}))\le\min\{\vol^{c}(V_{\ge i}),\vol^{c}(V_{<i})\}\cdot\frac{10\log C}{h}$.
Otherwise, $\vol^{c}(V_{\ge h/2})\ge(1+\frac{10\log C}{h})^{h/2}>2C$
which is a contradiction. We fix such $i$. Set $S=V_{\ge i}$. As
$0<i\le h$, so we have $|S|,|V\setminus S|>z$. We have, by \Cref{prop:cap
of skip}, that 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{i},V_{i-1}))+c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))\\
 & \le c(E(V_{i},V_{i-1}))+\Delta(V_{\ge i})+f(V_{i-i},V_{i})-\ab_{f}(V_{\ge i})-\ex_{f}(V_{\ge i})\\
 & <\Delta(S)-T(S)-z+c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i})).
\end{align*}
By the choice of $i$, we are done. 
\end{proof}

\subsubsection{Flow for Matching}

\label{sec:flow_for_matching}

The algorithm below is for computing approximate bipartite matching.
That is why the graph $G=(L,R,E)$ is bipartite and only has edges
from $L$ to $R$. The algorithm either send at least $\Delta(V)-z$
flow (i.e.~large fractional matching) or find a cut $S$ such that
the residual capacity is at most $2\frac{\Delta(V)-z}{h}$. So this
gives a $2/h$-approximation algorithm for bipartite matching. 
\begin{lem}
[Global Flow for Matchings]\label{lem:global flow matching}There
is a deterministic algorithm that, given a directed bipartite $m$-edge
graph $G=(V=(L,R),E)$ where $E\subseteq L\times R$, an excess parameter
$z\ge0$, a height parameter $h\ge1$, and a flow problem $\Pi=(\Delta,T,c)$
and the following holds 
\begin{enumerate}
\item $\Delta(R)=0$, $T(L)=0$, $\Delta(L)\le T(R)$, 
\item $\forall v\in V,\Delta(v),T(v)\le1$, 
\end{enumerate}
in $O(mh\log m)$ time, either 
\begin{itemize}
\item returns a preflow $f$ with total excess $\ex_{f}(L\cup R)\le z$,
or 
\item returns a set $S\subset V(G)$ where $|S|,|V\setminus S|>z$ and $c(E(S,V\setminus S))\le\Delta(S)-T(S)-z+2\cdot\frac{\Delta(V)-z}{h}$. 
\end{itemize}
\end{lem}

\begin{proof}
We call \Cref{prop: preflow and label} with parameter $h$ in $O(mh\log m)$.
Suppose that $\ex_{f}(V)>z$ otherwise we are done. By \Cref{prop:excess
give lower bound}, we know $|V_{h}|\ge\Delta(V_{h})>z$ and $|V_{0}|\ge T(V_{0})>z$
because $\forall v\in V,\Delta(v),T(v)\le1$. By \Cref{lem:bipartite
label}, $V_{h},V_{h-2},V_{h-4},\dots$ are subsets of $L$ and $V_{h-1},V_{h-3},V_{h-5},\dots$
are subsets of $R$. So $\sum_{i\ge1}f(V_{h-2i},V_{h-2i+1})\le f(L,R)\le\Delta(V)-z$.
So there is $1\le i\le h/2$ such that $f(V_{h-2i},V_{h-2i+1})\le2(\Delta(V)-z)/h$.
Fix such $i$ and set $S=V_{>h-2i}$. As $S\supseteq V_{h}$ and $S\cap V_{0}=\emptyset$
we have that $|S|,|V\setminus S|>z$. We have, by \Cref{prop:cap
of skip}, that 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{h-2i+1},V_{h-2i}))+c(E(V_{>h-2i},V_{\le h-2i})\setminus E(V_{h-2i+1},V_{h-2i}))\\
 & \le\Delta(V_{>h-2i})+f(V_{h-2i},V_{h-2i+1})-\ab_{f}(V_{>h-2i})-\ex_{f}(V_{>h-2i})\\
 & <\Delta(S)-T(S)-z+\frac{2(\Delta(V)-z)}{h}
\end{align*}
where the first inequality is because $E(V_{h-2i+1},V_{h-2i})=\emptyset$
as $V_{h-2i+1}\subset R$ and $V_{h-2i}\subset L$ and the second
inequality is by the choice of $i$. 
\end{proof}
This immediately implies the subroutine that we need in \Cref{sec:matching}.
We simply plug in the parameters correctly.

\MatchingOrCutLemma* 
\begin{proof}
W.l.o.g. we can assume that $|L|\le|R|$ and then we treat edges in
$G$ are directed edges from $L$ to $R$. Let $h=2/\epsilon$ and
$z=n-\mu(1-\epsilon)$. For each $v\in L$, let $\Delta(v)=1$ and
$T(v)=0$. For each $v\in R$, let $\Delta(v)=0$ and $T(v)=1$. Let
$\Pi=(\Delta,T,\kappa)$. We call the algorithm from \Cref{lem:global
flow matching} with $(G,z,h,\Pi)$ as input. Observe that the input
satisfies all the conditions of \Cref{lem:global flow matching}.

If \Cref{lem:global flow matching} returns a preflow $f$ with
excess at most $z$, then this means that we obtain a flow of size
at least $\Delta(V)-z=\mu(1-\epsilon)$ by \Cref{rem:excess at source
and path decomposition}. Obliviously, $f(e)\le\kappa(e)$ for all
$e$. If \Cref{lem:global flow matching} returns a set $S\subset V(G)$
such that $\kappa(E(S,V\setminus S))\le\Delta(S)-T(S)-z+2\cdot\frac{\Delta(V)-z}{h}$.
Let $S_{L}=S\cap L$ and $S_{R}=S\cap R$. Note that $\Delta(S)=|S_{L}|$,
$T(S)=|S_{R}|$, $\kappa(E(S,V\setminus S))=\kappa(S_{L},R\setminus S_{R})$,
and $2\frac{\Delta(V)-z}{h}-z=\epsilon\mu(1-\epsilon)-(n-\mu(1-\epsilon))=\mu(1-\epsilon^{2})-n.$
So we have 
\[
\kappa(S_{L},R\setminus S_{R})\le|S_{L}|-|S_{R}|+\mu-n
\]
as desired. 
\end{proof}

\subsubsection{Flow for Vertex Cuts}

\label{sec:flow_vertexcut}

The algorithm below is for finding sparse \emph{vertex cuts}.

\global\long\def\vv{\mathsf{v}}
 \global\long\def\vin{\mathrm{in}^{\vv}}
 \global\long\def\vout{\mathrm{out}^{\vv}}
\global\long\def\vertexflow{\textsc{VertexFlow}}

\SparseVertexCutLemma* 
\begin{proof}
For notational convenience, let us rename a graph that we want to
find a vertex cut as $G^{\vv}=(V^{\vv},E^{\vv})$ where $A,B\subset V^{\vv}$.
We use the standard reduction that splits each vertex into two vertices.
More precisely, we construct a bipartite graph $G=(V=(L,R),E)$ as
follows. For each vertex $v\in V^{\vv}$, we create $v_{L}\in L$
and $v_{R}\in R$ and add a directed edge $(v_{L},v_{R})$ with capacity
$\left\lfloor 1/\phi\right\rfloor $. For each each $(u,v)$, we add
a directed edge $(u_{R},v_{L})$ with capacity $\infty$. For $v\in A$,
we let $\Delta(v_{L})=1$. Set $\Delta(v)=0$ for all other vertices
in $G$. For each $v\in B$, we let $T(v_{R})=1$. Set $T(v)=0$ for
all other vertices in $G$. Let $c:E\rightarrow\mathbb{R}$ denote
the edge capacity of edges in $G$.

Let $\Pi$ be the integral flow problem on $G$ defined by $(\Delta,T,c)$.
We call \Cref{prop: preflow and label} with parameter $h=\frac{100\log(n/\phi)}{\phi}$
in $O(mh\log m)$ and obtain a preflow $f$ in $G$. Set $z=\epsilon|A|$.
There are two cases whether $\ex_{f}(V)\le z$ or not.

If $\ex_{f}(V)\le z$, then by \Cref{rem:excess at source and path
decomposition}, we can obtain a \emph{feasible} flow $\hat{f}$ in
$G$ with value at least $\Delta(V)-z=(1-\epsilon)|A|$. Moreover
we can obtain a path decomposition $\pset_{\hat{f}}$ of $\hat{f}$
in $O(\Delta(V)h)=O(nh)$ time. By reading the endpoint of paths in
$\pset_{\hat{f}}$, we obtain an integral matching $M$ of size at
least $(1-\epsilon)|A|$ from $A$ to $B$, such that $M$ can be
embedded into $G^{\vv}$ with vertex congestion $\left\lfloor 1/\phi\right\rfloor $.
This is because $\hat{f}$ corresponds to a flow in $G^{\vv}$ with
vertex congestion at most $\left\lfloor 1/\phi\right\rfloor $ by
the construction of $G$.

If $\ex_{f}(V)>z$, then by \Cref{prop:excess give lower bound},
we know $|V_{h}|\ge\Delta(V_{h})>z$ and $|V_{0}|\ge T(V_{0})>z$
because $\forall v\in V,\Delta(v),T(v)\le1$. By \Cref{lem:bipartite
label}, $V_{h},V_{h-2},V_{h-4},\dots$ are subsets of $L$ and $V_{h-1},V_{h-3},V_{h-5},\dots$
are subsets of $R$. Let $c'$ be an edge capacity function where
$c_{0}(e)=c(e)$ for all $e\in E(L,R)$ and $c_{0}(e)=0$ otherwise.
Let $C=\sum_{e\in E}c_{0}(e)=n\left\lfloor 1/\phi\right\rfloor $.
By the ball growing argument applying in two directions, there is
an index $0\le i<h/2$ such that $\vol^{c_{0}}(V_{h-2i})\le\min\{\vol^{c_{0}}(V_{\ge h-2i}),\vol^{c_{0}}(V_{<h-2i})\}\cdot\frac{20\log C}{h}$.
Otherwise, $\vol^{c_{0}}(V_{\ge h/2})\ge(1+\frac{20\log C}{h})^{h/2}>2C=\vol^{c_{0}}(V)$
which is a contradiction. Fix such $i$ and let $S=V_{\ge h-2i}$.
Now, we bound the cut size of $S$:
\begin{claim}
\label{claim:bound vertex cut} $c(E(S,V\setminus S))\le\Delta(S)-T(S)+2\vol^{c_{0}}(V_{h-2i})$.
In particular, $c(E(S,V\setminus S))$ is finite. 
\end{claim}

\begin{proof}
First, observe that the total mass flowing into $V_{h-2i}$ is at
most the total capacity of outgoing edges from $V_{h-2i}$ plus the
sink capacity of $V_{h-2i}$. That is, $f(V,V_{h-2i})\le c(E(V_{h-2i},V))+T(V_{h-2i-1})=c(E(V_{h-2i},V))$
where $T(V_{h-2i})=0$ as $V_{h-2i}\subseteq L$. In particular, we
have $f(V_{h-2i-1},V_{h-2i})\le c(E(V_{h-2i},V))$. Now, we have the
following: 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{h-2i},V_{h-2i-1}))+c(E(S,V\setminus S)\setminus E(V_{h-2i},V_{h-2i-1}))\\
 & \le c(E(V_{h-2i},V_{h-2i-1}))+\Delta(S)+f(V_{h-2i-1},V_{h-2i})-\ab_{f}(S)-\ex_{f}(S)\\
 & <\Delta(S)-T(S)-z+2c(E(V_{h-2i},V))\\
 & \le\Delta(S)-T(S)+2\vol^{c_{0}}(V_{h-2i})
\end{align*}
where the first inequality is by \Cref{prop:cap of skip}. The last
inequality follows because $V_{h-2i}\subseteq L$ and so $c(E(V_{h-2i},V))=c(E(V_{h-2i},R))=c_{0}(E(V_{h-2i},R))\le\vol^{c_{0}}(V_{h-2i})$. 
\end{proof}
Let $(X,Y,Z,F)$ be a partition of vertices $V^{\vv}$ in $G^{\vv}$
defined as follow: If $v_{L},v_{R}\in S$, then $v\in X$. If $v_{L}\in S$
and $v_{R}\notin S$, then $v\in Y$. If $v_{L},v_{R}\notin S$, then
$v\in Z$. If $v_{L}\notin S$ and $v_{R}\in S$, then $v\in F$.%

{} For any $U\subseteq V^{\vv}$, let $\vout(U)=\{v\notin U\mid\exists(u,v)\in E^{\vv}$
where $u\in U\}$ and $\vin(U)=\{v\notin U\mid\exists(v,u)\in E^{\vv}$
where $u\in U\}$ denote the set of out-neighbors and in-neighbors
of $U$ respectively.
\begin{claim}
\label{claim:vertex neighbor} We have $\vout(X)\subseteq Y$, $\vin(Z)\subseteq Y$,
$\vout(F)\subseteq X\cup Y$, and $\vin(F)\subseteq Z\cup Y$. 
\end{claim}

\begin{proof}
The idea of each of these four statements are the same. If it is not
true, then there is an edge $e\in E(R\cap S,L\setminus S)$, which
is impossible because $c(e)=\infty$ but $c(E(S,V\setminus S))$ is
finite. Now, we prove each statement one by one. 
\begin{itemize}
\item If $\vout(X)\not\subseteq Y$, then there is an edge $(x,u)$ in $G^{\vv}$
where $x\in X$ and $u\in Z\cup F$. So there is an edge $(x_{R},u_{L})$
in $G$ which is from $E_{G}(R\cap S,L\setminus S)$. 
\item If $\vin(Z)\not\subseteq Y$, then there is an edge $(u,z)$ in $G^{\vv}$
where $u\in X\cup F$ and $z\in Z$. So there is an edge $(u_{R},z_{L})$
in $G$ which is from $E_{G}(R\cap S,L\setminus S)$. 
\item If $\vout(F)\not\subseteq X\cup Y$, then there is an edge $(f,u)$
in $G^{\vv}$ where $f\in F$ and $u\in Z$. So there is an edge $(f_{R},u_{L})$
in $G$ which is from $E_{G}(R\cap S,L\setminus S)$. 
\item If $\vin(F)\not\subseteq Z\cup Y$, then there is an edge $(u,f)$
in $G^{\vv}$ where $u\in X$ and $f\in F$. So there is an edge $(u_{R},f_{L})$
in $G$ which is from $E_{G}(R\cap S,L\setminus S)$. 
\end{itemize}
\end{proof}
Now, we can define a vertex cut in $G^{\vv}$ that we will output.
Partition $F$ into two halves $F_{x},F_{z}$. Our output is $(X\cup F_{x},Y,Z\cup F_{z})$.
From \Cref{claim:vertex neighbor}, observe that $(X\cup F_{x},Y,Z\cup F_{z})$
is a vertex cut in $G^{\vv}$ because $E^{\vv}(X\cup F_{x},Z\cup F_{z})=\emptyset$.
As both $|F_{x}|,|F_{z}|\ge|F|/3$, the following claim implies that
$(X\cup F_{x},Y,Z\cup F_{z})$ is $O(\phi)$-vertex-sparse:
\begin{claim}
$|Y|\le O(\phi)\cdot\min\{|X\cup F|,|Z\cup F|\}$. 
\end{claim}

\begin{proof}
Recall that $\vol^{c_{0}}(V_{h-2i})\le\min\{\vol^{c_{0}}(V_{\ge h-2i}),\vol^{c_{0}}(V_{<h-2i})\}\cdot\frac{20\log C}{h}$
by the choice of $i$. Now, observe that $\vol^{c_{0}}(V_{\ge h-2i})=\vol^{c_{0}}(S)=(2|X|+|Y|+|F|)\cdot\left\lfloor 1/\phi\right\rfloor $,
and $\vol^{c_{0}}(V_{<h-2i})=\vol^{c_{0}}(V\setminus S)=(2|Z|+|Y|+|F|)\cdot\left\lfloor 1/\phi\right\rfloor $.
Also, $c(E(S,V\setminus S))=|Y|\cdot\left\lfloor 1/\phi\right\rfloor $,
$\Delta(S)=|X|+|Y|$ and $T(S)=|X|+|F|$. Recall that $h=\frac{100\log(n/\phi)}{\phi}$,
so we have the following by \Cref{claim:bound vertex cut}: 
\begin{align*}
|Y|\cdot\left\lfloor 1/\phi\right\rfloor  & \le(|X|+|Y|)-(|X|+|F|)+\min\{2|X|+|Y|+|F|,2|Z|+|Y|+|F|\}\cdot\left(2\cdot\left\lfloor 1/\phi\right\rfloor \cdot\frac{20\log(n/\phi)}{(\frac{100\log(n/\phi)}{\phi})}\right)\\
 & \le|Y|+\min\{|X|+|Y|+|F|,|Z|+|Y|+|F|\}.
\end{align*}
So $|Y|(\left\lfloor 1/\phi\right\rfloor -2)\le\min\{|X\cup F|,|Z\cup F|\}$
and so $|Y|\le O(\phi)\cdot\min\{|X\cup F|,|Z\cup F|\}$. 
\end{proof}
It remains to show that $(X\cup F_{x},Y,Z\cup F_{z})$ is $\Omega(\epsilon)$-vertex-balanced.
Observe that $|X\cup Y\cup F|\ge|S|>z$ and $|Z\cup Y\cup F|\ge|V\setminus S|>z$.
As we have $|Y|\le O(\phi)\cdot\min\{|X\cup F|,|Z\cup F|\}$, so $|X\cup F_{x}|,|Z\cup F_{z}|=\Omega(z)=\Omega(\epsilon n)$
by assuming that $\phi$ is smaller than a constant. 
\end{proof}



==> flow_old.tex <==

\section{Implementation of Flow Subroutines}

\label{sec:flow}

Throughout this paper, we use several flow subroutines for various
contexts (e.g.~expander pruning, embedding robust witness, finding
approximate matching, etc.). All these flow algorithms are based on
the same techniques which is the \emph{bounded height variant} of
push-relabel and blocking flow algorithms. This idea was used explicitly
many times before (e.g.~\cite{LangR04,OrecchiaZ14,HenzingerRW17,SaranurakW19}).
Our contribution in this section is only to show a uniform presentation
that all of our flow subroutines can be implemented using the same
framework, and to give proofs for completeness.

We start with introducing notations in \Cref{sec:flow notation}, then
we describe the guarantee of the bounded height variant of push-relabel
and blocking flow algorithms in \Cref{sec:bounded height flow}. All
the flow subroutines share the same framework which is described in
\Cref{sec:flow framework}. Using this framework, we instantiate the
flow subroutines that we need throughout the paper in \Cref{sec:flow subroutine}.

\subsection{Flow Notations}

\label{sec:flow notation}

The notation below is slight adjusted from \cite{SaranurakW19} because
we work with directed graphs instead of undirected graph. 

A \emph{flow problem} $\Pi$ on a \emph{directed} graph $G=(V,E)$
is specified by a source function $\Delta:V\rightarrow\mathbb{R}_{\geq0}$,
a sink capacity function $T:V\rightarrow\mathbb{R}_{\geq0}$, and
edge capacities $c:E\rightarrow\mathbb{R}_{\geq0}$. We say that $\Pi$
is \emph{integral} if $\Delta:V\rightarrow\mathbb{Z}_{\geq0}$, $T:V\rightarrow\mathbb{Z}_{\geq0}$,
and $c:E\rightarrow\mathbb{Z}_{\geq0}$. More generally, for any number
$d\ge1$, we say that $\Pi$ is $1/d$-integral if $\Delta:V\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$,
$T:V\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$, and $c:E\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$.
We use \emph{mass} to refer to the substance being routed. For a vertex
$v$, $\Delta(v)$ specifies the amount of mass initially placed on
$v$, and $T(v)$ specifies the capacity of $v$ as a sink. For an
edge $e$, $c(e)$ bounds how much mass can be routed along the edge.

A \emph{routing} (or \emph{flow}) $f:E\rightarrow\mathbb{R}_{\ge0}$
is $1/d$-integral if $f:E\rightarrow\frac{1}{d}\mathbb{Z}_{\geq0}$.
$f(u,v)>0$ means that mass is routed in the direction from $u$ to
$v$. If $f(u,v)=c(u,v)$, then we say $(u,v)$ is \emph{saturated}.
Given $\Delta$, we also treat $f$ as a function on vertices, where
$f(v)=\Delta(v)+\sum_{u}f(u,v)$ is the amount of mass ending at $v$
after the routing $f$. If $f(v)\ge T(v)$, then we say $v$'s sink
is \emph{saturated}. For $A,B\subset V$, let $f(A,B)=\sum_{(u,v)\in E\cap(A\times B)}f(u,v)$
be the total mass routing directly from $A$ to $B$. 

We say that $f$ is a \emph{feasible routing/flow} for $\Pi$ if $f(u,v)\leq c(u,v)$
for each edge $e=(u,v)$ (i.e.~obey edge capacities), $\sum_{u}f(v,u)\leq\Delta(v)$
for each $v$ (i.e.~the net amount of mass routed away from a vertex
can be at most the amount of its initial mass), and $f(v)\leq T(v)$
for each $v$ (i.e.~no excess flow on each vertex). 

Given a flow problem $\Pi=(\Delta,T,c)$, a \emph{pre-flow} $f$ is
a feasible routing for $\Pi$ except the condition $\forall v:f(v)\leq T(v)$
may not be satisfied. As pre-flow may not obey sink capacity on vertices,
we define the \emph{absorbed} mass on a vertex $v$ as $\ab_{f}(v)=\min(f(v),T(v))$.
We have $\ab_{f}(v)=T(v)$ iff $v$'s sink is saturated. The \emph{excess}
on $v$ is $\ex_{f}(v)=f(v)-\ab_{f}(v)$. From the definition, when
there is no excess, $\forall v:\ex_{f}(v)=0$, then $f$ is a feasible
flow for $\Pi$. Intuitively, we think of $\Delta(v)-T(v)$ as \emph{initial
excess} at $v$, and $\ex_{f}(v)$ is the excess at $v$ after routing
$f$. Similarly, we think of $\min\{\Delta(v),T(v)\}$ as \emph{initial
absorbed mass} at $v$ and $\ab_{f}(v)$ is the absorbed mass at $v$
after routing $f$. For any $S\subseteq V$, we usually write $x(S)=\sum_{v\in S}x(v)$
where $x$ can be from $\{\Delta,T,\ex_{f},\ab_{f}\}$ (e.g.~$\Delta(S)$,
$\ab_{f}(S)$). We omit the subscript whenever it is clear. 

For any directed path $P$, let $|P|$ denote the number of edges
in $P$. A \emph{path-decomposition} of a pre-flow $f$ is a collection
$\pset_{f}$ of directed paths with \emph{value} $\val(P)>0$ associated
with each path $P\in\pset_{f}$ and $\sum_{P\in\pset_{f}\mid P\ni e}\val(P)=f(e)$
for all $e\in E$.

\subsection{Bounded Height Push-Relabel and Blocking Flow}

\label{sec:bounded height flow}

The following proposition is the key algorithmic component for the
whole section. 
\begin{prop}
\label{prop: preflow and label}There is an algorithm that, given
a directed $n$-vertex $m$-edge graph $G=(V,E)$, a height parameter
$h\ge1$, and a flow problem $\Pi=(\Delta,T,c)$, returns a preflow
$f$ together with labels on vertices $l:V\rightarrow\{0,\dots,h\}$
such that:
\begin{enumerate}
\item \label{enu:cross for}If $l(u)>l(v)+1$ and $(u,v)\in E$, then the
mass on $(u,v)$ is saturated, i.e.,~$f(u,v)=c(u,v)$.
\item \label{enu:cross back}If $l(u)>l(v)+1$ and $(v,u)\in E$, then the
mass on $(v,u)$ is empty, i.e.,~$f(v,u)=0$.
\item \label{enu:no excess}If $l(v)<h$, then $v$ has no excess, i.e.~$\ex_{f}(v)=0$.
\item \label{enu:full absorb}If $l(v)>0$, then $v$'s sink is saturated,
i.e.~$\ab_{f}(v)=T(v)$.
\item \label{enu:monotone}After routing $f$, excess does not increase
and absorbed mass never decreases, i.e.~$\ex_{f}(v)\le\max\{\Delta(v)-T(v),0\}$
and $\ab_{f}(v)\ge\min\{\Delta(v),T(v)\}$ for all $v$.
\end{enumerate}
The algorithm takes at most $O(mh\log m)$ time. If $\Pi$ is $1/d$-integral
for some number $d\ge1$, then so is $f$. If $\Pi$ is integral,
$T(v)\ge\deg(v)$ for all $v\in V$, and the algorithm can access
the adjacency list of every vertex, then the running time can be reduced
to $O(\Delta(V)h)$.
\end{prop}

\begin{proof}
The statement simply summarizes the output that one can obtain from
performing blocking flow computations for $\approx h$ rounds (instead
of $\approx n$ rounds as when we want to solve the exact max flow
problem). 

We explain this idea in more detail. Let us create a graph $G'$ from
the graph $G$ by adding a super source vertex $s$ and a super sink
vertex $t$. For each $u\in V$, we add an edge $(s,u)$ with capacity
$\Delta(u)$. For each $u\in V$, we add an edge $(u,t)$ with capacity
$T(u)$. Then, we run blocking flow for at most $h+2$ rounds until
the (unweighted) distance between $s$ and $t$ in the residual graph
$G'_{f}$ of $G'$ is at least $h+2$. Each blocking flow computation
takes $O(m\log m)$ time (even when the flow problem $\Pi$ is fractional).
This running time is possible by using the \emph{link-cut tree data
structure}. (See the detail in Section 6 of \cite{SleatorT83}, Page
387-389.) So the total running time is $O(mh\log m)$. This completes
the running time analysis.

Let $f$ be the flow in $G'$ obtained after the blocking flow computations.
We can define the vertex labeling $l:V\cup\{s,t\}\rightarrow\{0,\dots,h\}$
as follows. For $0\le i\le h$, we set $l(u)=h-i+1$ where $i$ is
the (unweighted) distance between $s$ and $u$ in $G'_{f}$. For
all vertices $u$ whose distance from $s$ is more than $h$, we set
$l(u)=0$. By definition, $l(s)=h+1$. Also, as the distance from
$s$ to $t$ in $G'_{f}$ is $h+2$, for each label $i\in\{0,\dots,h\}$,
there must exist a vertex with label $i$. Observe that, for any edge
$(u,v)$ where $|l(u)-l(v)|>1$, the residual capacity in $G'_{f}$
must be $c_{f}(u,v)=0$. So this implies \Cref{enu:cross for} and
\Cref{enu:cross back}. 

Note that we can view $f$ as a preflow on $G$ by restricting $f$
to only edges of $G$. Observe that the flow value on $(u,t)$ in
$G'$ corresponds to the absorbed flow at $u$ in $G$, i.e.~$f(u,t)=\ab_{f}(u)$.
Also, the residual capacity $c_{f}(s,u)$ of $(s,u)$ in $G'_{f}$
corresponds to the excess at $u$ after routing $f$, i.e.~$c_{f}(s,u)=\Delta(u)-f(s,u)=\ex_{f}(u)$.
So if $l(u)<h$, then $c_{f}(s,u)=0$ and so $\ex_{f}(u)=0$. Also,
if $l(u)>0$, then $c_{f}(u,t)=0$ and so $\ab_{f}(u)=T(u)$. This
implies \Cref{enu:no excess} and \Cref{enu:full absorb}. 

In fact, our algorithm will do some simple preprocessing. For each
$u$, we will assume that we start with the initial flow that go through
$(s,u)$ and $(u,t)$ with value $\min\{\Delta(u),T(u)\}$. So initially there are $\min\{\Delta(u),T(u)\}$ unit of mass absorbed at $u$
and the initial excess at $u$ is $\max\{\Delta(u)-T(u),0\}$. As
the blocking flow computations have a property that flow value incident
to $s$ and $t$ never decreases. This implies \Cref{enu:monotone}.
This completes the correctness of the algorithm with running time
$O(mh\log m)$. Note that the implementation of blocking flow using
link-cut tree also have the guarantee that flow value on each edge
is $1/d$-integral if the given flow problem $\Pi$ is $1/d$-integral. 

Lastly, we need to show if $\Pi$ is integral, $T(v)\ge\deg(v)$ for
all $v\in V$, and the algorithm can access the adjacency list of
every vertex, then the running time is $O(\Delta(V)h)$. However,
the proposition here is simply the summary of the output by the Unit
Flow algorithm by Henzinger Rao and Wang \cite{HenzingerRW17} (see
also \cite{SaranurakW19}) where Unit Flow is a bounded height variant
of push-relabel algorithms.
\end{proof}
\begin{lem}
\label{lem:path decomposition}Given a preflow $f$ from the algorithm
from \Cref{prop: preflow and label}, any path decomposition $\pset_{f}$
of $f$ satisfies $\sum_{P\in\pset_{f}}\val(P)|P|\le\Delta(V)h$.
Moreover, if the flow problem $\Pi$ is $1/d$-integral, then a decomposition
$\pset_{f}$ can be computed in time $O(\sum_{P\in\pset_{f}}|P|)=O(d\Delta(V)h)$. 
\end{lem}

\begin{proof}
By the definition of path decomposition, we have $\sum_{P\in\pset_{f}\mid P\ni e}\val(P)=f(e)$
for all $e\in E$. So 
\[
\sum_{P\in\pset_{f}}\val(P)|P|=\sum_{e\in E}\sum_{P\in\pset_{f}\mid P\ni e}\val(P)=\sum_{e\in E}f(e).
\]
Now, we want to show that $\sum_{e\in E}f(e)\le\Delta(V)h$. Consider
the bounded height blocking-flow algorithm or push-relabel algorithm.
The algorithm always sends the flow along a path of length at most
$h$ in the residual graph. So even the total flow value over all
edges ``without flow cancellation'' must be at most $\Delta(V)h$.
As $\sum_{e\in E}f(e)$ is the total flow value over all edges ``after
flow cancellation'', we conclude that $\sum_{e\in E}f(e)\le\Delta(V)h$.

We can find a path decomposition $\pset_{f}$ of a flow $f$ in time
$O(\sum_{P\in\pset_{f}}|P|)$ as follows. As the flow problem $\Pi$
is $1/d$-integral, the flow value of each edge $f(e)$ is also $1/d$-integral
by \Cref{prop: preflow and label}. Let $H$ be a graph induced by
edges $e$ where positive flow value $f(e)>0$. We make $H$ unweighted
by scaling up all edges in $H$ by a factor of $d$. Then, we add
a dummy source to $H$ and performing the depth-first search on $H$
from the dummy source. Whenever a search reaches a sink $u$ (i.e.
$\ab_{f}(u)>0$) or the search cannot proceed from $u$ (i.e. $\ex_{f}(u)>0$),
we backtrack and output the corresponding path $P$ excluding the
dummy source. Note that $P$ is a directed \emph{simple} path in $H$ and corresponds
to a flow path of value $1/d$. We remove the path $P$ from $H$
and repeat. 

Observe that each edge in $H$ is read at most twice and so the total
time is subsumed by the total time for outputting all paths which
is $O(\sum_{P\in\pset_{f}}|P|)$. As $\val(P)\ge1/d$, so $O(\sum_{P\in\pset_{f}}|P|)\le O(\sum_{P\in\pset_{f}}d\cdot\val(P)|P|)=O(d\Delta(V)h)$.
\end{proof}
For convenience, we will use the following notation throughout this
section.
\begin{defn}
Given a vertex labeling $l:V\rightarrow\{0,\dots,h\}$, let $V_{i}=\{u\mid l(u)=i\}$
for each $i$. Also, we define $V_{\ge i}=\{u\mid l(u)\ge i\}$ and
$V_{>i},V_{\le i},V_{<i}$ are defined similarly. 
\end{defn}
When the input graph to \Cref{prop: preflow and label} is bipartite
and all source/sink vertices are only on the left/right respectively,
we can additionally guarantee that the vertices from each level alternate
between the left and right side of the bipartite graph $G$. 
\begin{lem}
\label{lem:bipartite label}If the input graph from \Cref{prop: preflow and label}
is a bipartite graph $G=(L,R,E)$ where $R$ has no initial mass ($\Delta(R)=0$),
and $L$ cannot absorb mass ($T(L)=0$), then the vertex labeling
$l$ from \Cref{prop: preflow and label} has additional property that
$V_{h},V_{h-2},V_{h-4},\dots\subseteq L$ and $V_{h-1},V_{h-3},V_{h-5},\dots\subseteq R$. 
\end{lem}

\begin{proof}
This guarantee follows immediately when we use blocking-flow-based
algorithms. For Unit Flow (push-relabel-based algorithm), we can guarantee
this using very simple modification: we initialize by assigning all
all vertices in $L$ a label $1$ and all vertices in $R$ a label
$0$, and when ever we relabel a vertex $l(u)\gets l(u)+1$, we instead
set $l(u)\gets l(u)+2$. All the invariants of the push-relabel-based
algorithm will still be maintained because the graph is bipartite.
\end{proof}

\subsection{The Common Framework}

\label{sec:flow framework}

Given a flow problem $\Pi=(\Delta,T,c)$ for a graph $G=(V,E)$, all
the algorithms in \Cref{sec:flow subroutine} starts by calling \Cref{prop: preflow and label}
with parameter $h$ and obtain a preflow $f$ and a vertex labeling
$l:V\rightarrow\{0,\dots h\}$. 

If the total excess after routing $f$ is at most $z$, then the algorithm
just returns $f$ and we are done%

. Otherwise, the algorithm will return one of the \emph{level-$i$
cuts} $(V_{\ge i},V_{<i})$ for some $0<i\le h$. The only main task
we need to prove in each algorithm is to show that there exists an
index $i$ such that the level-$i$ cut satisfies the requirement
of the lemma.

There are two common arguments that will be used by all flow algorithms
in \Cref{sec:flow subroutine}. The first one will be used to lower
bound the ``size'' of both $V_{h}$ and $V_{0}$ by the total excess.
In our algorithm, the outputted cut $S$ will be such that $S\supset V_{h}$
and $S\cap V_{0}=\emptyset$, so the proposition below will be useful
to prove the balance of $(S,V\setminus S)$.
\begin{prop}
\label{prop:excess give lower bound}If $\Delta(V)\le T(V)$, then
$\Delta(V_{h})\ge\ex_{f}(V)$ and $T(V_{0})\ge\ex_{f}(V)$.
\end{prop}

\begin{proof}
First, note that $\ex_{f}(V)=\ex_{f}(V_{h})$ because all vertices
with level below $h$ has no excess by \Cref{enu:no excess} of \Cref{prop: preflow and label}.
Also, $\ex_{f}(V_{h})\le\Delta(V_{h})-T(V_{h})$ because excess does
not increase (\Cref{enu:monotone} of \Cref{prop: preflow and label}).
So $\ex_{f}(V)\le\Delta(V_{h})$. Similarly, First, note that $T(V_{0})-\ab_{f}(V_{0})=T(V)-\ab_{f}(V)$
because all vertices with level above $0$ are fully absorbed by \Cref{enu:full absorb}
of \Cref{prop: preflow and label}. Also, we have $T(V)-\ab_{f}(V)\ge\Delta(V)-\ab_{f}(V)=\ex_{f}(V)$
by the assumption that $T(V)\ge\Delta(V)$ and by the definition of
$\ex_{f}(V)$. So $\ex_{f}(V)\le T(V_{0})$.
\end{proof}
The next common argument is for upper bounding the total capacity
of the level cut $(V_{\ge i},V_{<i})$. The argument used for bounding
capacity of ``consecutive-level'' edges from $E(V_{i},V_{i-1})$
will be different in each algorithm. But, the argument for bounding
total capacity of edges that are not from $E(V_{i},V_{i-1})$ will
be the same and is stated as follow:
\begin{prop}
\label{prop:cap of skip}$c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))\le\Delta(V_{\ge i})+f(V_{i-i},V_{i})-\ab_{f}(V_{\ge i})-\ex_{f}(V_{\ge i})$.
\end{prop}

\begin{proof}
First, note that each $(u,v)\in E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1})$
is ``skipping levels'', i.e.~$l(u)-l(v)>1$. So, by \Cref{enu:cross for}
of \Cref{prop: preflow and label}, we have $f(u,v)=c(u,v)$. So the
total capacity $c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))$
is at most the total mass going out of $V_{\ge i}$. Observe that
the total mass in-coming into $V_{\ge i}$ is $f(V_{i-i},V_{i})$
because any other edges $(u,v)\in E(V_{<i},V_{\ge i})\setminus E(V_{i-i},V_{i})$
is ``skipping levels'' and so $f(u,v)=0$ by \Cref{enu:cross back}
of \Cref{prop: preflow and label}. Therefore, the total mass going
out of $V_{\ge i}$ is at most 
\begin{align*}
\underset{\textrm{initial mass}}{\underbrace{\Delta(V_{\ge i})}}+\underset{\textrm{incoming mass}}{\underbrace{f(V_{i-i},V_{i})}}-\underset{\textrm{absorbed mass}}{\underbrace{\ab_{f}(V_{\ge i})}}-\underset{\textrm{excess}}{\underbrace{\ex_{f}(V_{\ge i})}}
\end{align*}
\end{proof}

\subsection{Flow Subroutines}

\label{sec:flow subroutine}

In this section, we state the flow subroutines that will be used by
several places throughout our paper. To state some lemmas below, we
also define degree and volume w.r.t. capacity function $c$. Given
a graph $G=(V,E)$ with edge capacity $c$, for $u\in V$, let $\deg^{c}(u)=\sum_{(u,v)}c(u,v)+\sum_{(v,u)}c(v,u)$
denote the weighted degree w.r.t.~$c$. For $S\subset V$, let $\vol^{c}(S)=\sum_{u\in S}\deg^{c}(u)$
be the volume of $S$ w.r.t.~$c$. 

The following remark will be used repeatedly.
\begin{rem}
\label{rem:excess at source and path decomposition}
Let $f$ be a preflow returned by any of the algorithms below in this section. 
Note that every algorithm below starts by calling the algorithm from \Cref{prop: preflow and label} with parameter $h$ on some graph.
Note that any vertex $\ex_{f}(v)>0$ with positive excess must have positive initial excess, i.e.~$\Delta(v)-T(v)>0$. 
This follows from \Cref{enu:monotone} of \Cref{prop: preflow and label}.
By simply scanning vertices with initial excess and removing excess after routing $f$, we obtain a \emph{feasible flow} $f'$ of value $\Delta(V) - \ex_{f}(v)$ from $f$. The time to remove these excess is obviously subsumed by the algorithm because the algorithm at least need to read all vertices with initial excess.
Moreover, we can obtain a path decomposition of $f$ in additional time $O(d\Delta(V)h)$ if the flow problem is $1/d$-integral by  \Cref{lem:path decomposition}.
\end{rem}

\subsubsection{Local Flow}

The algorithm below either sends most of the flow or finds a balanced
sparse cut in \emph{local} time. We need that the given flow problem
is integral and each vertex can absorb mass at least by its degree.
\begin{lem}
[Local Flow]\label{lem:local flow}There is a deterministic
algorithm that, given access to the adjacency list of every vertex
of a directed $m$-edge graph $G=(V,E)$, parameters $z\ge0$ and
$h\ge1$, and an \emph{integral} flow problem $\Pi=(\Delta,T,c)$
with total capacity $C=\sum_{e\in E}c(e)$ where 
\begin{enumerate}
\item $\forall v,\Delta(v)\le\overline{\Delta}\deg(v)$ and $T(v)\ge\deg(v)$ where $\deg(v)$ denote an unweighted degree of $v$ in $G$.
\end{enumerate}
in $O(\Delta(V)\cdot h)$ time either 
\begin{itemize}
\item returns a preflow $f$ with total excess $\ex_{f}(V)\le z$, or
\item returns a set $S$ where $z/\overline{\Delta}<\vol(S)\le\Delta(V)$
and $c(E(S,V\setminus S))\le\Delta(S)-T(S)-z+\vol^{c}(S)\cdot\frac{10\log C}{h}$.
\end{itemize}
\end{lem}

\begin{proof}
We call \Cref{prop: preflow and label} with parameter $h$. By the
assumption of the lemma, the running time is $O(\Delta(V)h)$. Suppose
that $\ex_{f}(V)>z$ otherwise we are done. By \Cref{prop:excess give lower bound},
we know $\vol(V_{h})\overline{\Delta}\ge\Delta(V_{h})>z$ because
$\forall v\in V,\Delta(v)\le\overline{\Delta}\deg(v)$. So $\vol(V_{h})>z/\overline{\Delta}$.
Also, observe that $\vol(V_{\ge1})\le\Delta(V)$. This is because
all vertices in $V_{\ge1}$ are fully absorbed by \Cref{enu:full absorb}
of \Cref{prop: preflow and label}, so $T(V_{\ge1})\le\ab_{f}(V_{\ge1})\le\Delta(V)$,
and because $T(V_{\ge1})\ge\vol(V_{\ge1})$ as $T(v)\ge\deg(v)$ for
all $v$.

By the ball growing argument, there is an index $0<i\le h$ such that
$c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i}))\le\min\{\vol^{c}(V_{\ge i}),\vol^{c}(V_{<i})\}\cdot\frac{10\log C}{h}$.
Otherwise, $\vol^{c}(V_{\ge1})\ge(1+\frac{10\log C}{h})^{h}>2C$ which
is a contradiction. We fix such $i$. Set $S=V_{\ge i}$. As $0<i\le h$,
so we have $z/\overline{\Delta}<\vol(S)\le\Delta(V)$. We have, by
\Cref{prop:cap of skip}, that 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{i},V_{i-1}))+c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))\\
 & \le c(E(V_{i},V_{i-1}))+\Delta(V_{\ge i})+f(V_{i-i},V_{i})-\ab_{f}(V_{\ge i})-\ex_{f}(V_{\ge i})\\
 & <\Delta(S)-T(S)-z+c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i})).
\end{align*}
By the choice of $i$, we are done.
\end{proof}

\subsubsection{Global Flow}

The algorithm below either sends most of the flow or finds a balanced
sparse cut when the flow problem is fractional. This is needed because
the capacity of edges will be fractional when we maintain the robust
witness.
\begin{lem}
[Global Flow]\label{lem:global flow}There
is a deterministic algorithm that, given a directed $m$-edge graph
$G=(V,E)$, excess parameter $z\ge0$, a height parameter $h\ge1$,
and a flow problem $\Pi=(\Delta,T,c)$ with total capacity $C=\sum_{e\in E}c(e)$
where 
\begin{enumerate}
\item $\Delta(V)\le T(V)$, 
\item $\forall v\in V,\Delta(v),T(v)\le1$,
\end{enumerate}
in $O(mh\log m)$ time, either 
\begin{itemize}
\item returns a preflow $f$ with total excess $\ex_{f}(V)\le z$, or
\item returns a set $S\subset V$ where $|S|,|V\setminus S|>z$ and $c(E(S,V\setminus S))\le\Delta(S)-T(S)-z+\min\{\vol^{c}(S),\vol^{c}(V\setminus S)\}\cdot\frac{10\log C}{h}$.
\end{itemize}
\end{lem}

\begin{proof}
We call \Cref{prop: preflow and label} with parameter $h$ in $O(mh\log m)$.
Suppose that $\ex_{f}(V)>z$. By \Cref{prop:excess give lower bound},
we know $|V_{h}|\ge\Delta(V_{h})>z$ and $|V_{0}|\ge T(V_{0})>z$
because $\forall v\in V,\Delta(v),T(v)\le1$. By the ball growing
argument applying in two directions, there is an index $0<i\le h$
such that $c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i}))\le\min\{\vol^{c}(V_{\ge i}),\vol^{c}(V_{<i})\}\cdot\frac{10\log C}{h}$.
Otherwise, $\vol^{c}(V_{\ge h/2})\ge(1+\frac{10\log C}{h})^{h/2}>2C$
which is a contradiction. We fix such $i$. Set $S=V_{\ge i}$. As
$0<i\le h$, so we have $|S|,|V\setminus S|>z$. We have, by \Cref{prop:cap of skip},
that 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{i},V_{i-1}))+c(E(V_{\ge i},V_{<i})\setminus E(V_{i},V_{i-1}))\\
 & \le c(E(V_{i},V_{i-1}))+\Delta(V_{\ge i})+f(V_{i-i},V_{i})-\ab_{f}(V_{\ge i})-\ex_{f}(V_{\ge i})\\
 & <\Delta(S)-T(S)-z+c(E(V_{i},V_{i-1})\cup E(V_{i-1},V_{i})).
\end{align*}
By the choice of $i$, we are done.
\end{proof}


\subsubsection{Flow for Matching}
\label{sec:flow_for_matching}

The algorithm below is for computing approximate bipartite matching.
That is why the graph $G=(L,R,E)$ is bipartite and only has edges
from $L$ to $R$. The algorithm either send at least $\Delta(V)-z$
flow (i.e.~large fractional matching) or find a cut $S$ such that
the residual capacity is at most $2\frac{\Delta(V)-z}{h}$. So this
gives a $2/h$-approximation algorithm for bipartite matching.
\begin{lem}
[Global Flow for Matchings]\label{lem:global flow matching}There
is a deterministic algorithm that, given a directed bipartite $m$-edge
graph $G=(V=(L,R),E)$ where $E\subseteq L\times R$, an excess parameter
$z\ge0$, a height parameter $h\ge1$, and a flow problem $\Pi=(\Delta,T,c)$
and the following holds
\begin{enumerate}
\item $\Delta(R)=0$, $T(L)=0$, $\Delta(L)\le T(R)$, 
\item $\forall v\in V,\Delta(v),T(v)\le1$, 
\end{enumerate}
in $O(mh\log m)$ time, either 
\begin{itemize}
\item returns a preflow $f$ with total excess $\ex_{f}(L\cup R)\le z$, or
\item returns a set $S\subset V(G)$ where $|S|,|V\setminus S|>z$ and $c(E(S,V\setminus S))\le\Delta(S)-T(S)-z+2\cdot\frac{\Delta(V)-z}{h}$.
\end{itemize}
\end{lem}

\begin{proof}
We call \Cref{prop: preflow and label} with parameter $h$ in $O(mh\log m)$.
Suppose that $\ex_{f}(V)>z$ otherwise we are done. By \Cref{prop:excess give lower bound},
we know $|V_{h}|\ge\Delta(V_{h})>z$ and $|V_{0}|\ge T(V_{0})>z$
because $\forall v\in V,\Delta(v),T(v)\le1$. By \Cref{lem:bipartite label},
$V_{h},V_{h-2},V_{h-4},\dots$ are subsets of $L$ and $V_{h-1},V_{h-3},V_{h-5},\dots$
are subsets of $R$. So $\sum_{i\ge1}f(V_{h-2i},V_{h-2i+1})\le f(L,R)\le\Delta(V)-z$.
So there is $1\le i\le h/2$ such that $f(V_{h-2i},V_{h-2i+1})\le2(\Delta(V)-z)/h$.
Fix such $i$ and set $S=V_{>h-2i}$. As $S\supseteq V_{h}$ and $S\cap V_{0}=\emptyset$
we have that $|S|,|V\setminus S|>z$. We have, by \Cref{prop:cap of skip},
that 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{h-2i+1},V_{h-2i}))+c(E(V_{>h-2i},V_{\le h-2i})\setminus E(V_{h-2i+1},V_{h-2i}))\\
 & \le\Delta(V_{>h-2i})+f(V_{h-2i},V_{h-2i+1})-\ab_{f}(V_{>h-2i})-\ex_{f}(V_{>h-2i})\\
 & <\Delta(S)-T(S)-z+\frac{2(\Delta(V)-z)}{h}
\end{align*}
where the first inequality is because $E(V_{h-2i+1},V_{h-2i})=\emptyset$
as $V_{h-2i+1}\subset R$ and $V_{h-2i}\subset L$ and the second
inequality is by the choice of $i$.
\end{proof}

This immediately implies the subroutine that we need in \Cref{sec:matching}. We simply plug in the parameters correctly.

\MatchingOrCutLemma*
\begin{proof}
	W.l.o.g. we can assume that $|L|\le|R|$ and then we treat edges in
	$G$ are directed edges from $L$ to $R$. Let $h=2/\epsilon$ and
	$z=n-\mu(1-\epsilon)$. For each $v\in L$, let $\Delta(v)=1$ and
	$T(v)=0$. For each $v\in R$, let $\Delta(v)=0$ and $T(v)=1$. Let
	$\Pi=(\Delta,T,\kappa)$. We call the algorithm from \Cref{lem:global flow matching}
	with $(G,z,h,\Pi)$ as input. Observe that the input satisfies all
	the conditions of \Cref{lem:global flow matching}. 
	
	If \Cref{lem:global flow matching} returns a preflow $f$ with excess
	at most $z$, then this means that we obtain a flow of size at least
	$\Delta(V)-z=\mu(1-\epsilon)$ by \Cref{rem:excess at source and path decomposition}. Obliviously, $f(e) \le \kappa(e)$ for all $e$.
	If \Cref{lem:global flow matching} returns a set $S\subset V(G)$
	such that $\kappa(E(S,V\setminus S))\le\Delta(S)-T(S)-z+2\cdot\frac{\Delta(V)-z}{h}$.
	Let $S_{L}=S\cap L$ and $S_{R}=S\cap R$. Note that $\Delta(S)=|S_{L}|$,
	$T(S)=|S_{R}|$, $\kappa(E(S,V\setminus S))=\kappa(S_{L},R\setminus S_{R})$,
	and $2\frac{\Delta(V)-z}{h}-z=\epsilon\mu(1-\epsilon)-(n-\mu(1-\epsilon))=\mu(1-\epsilon^{2})-n.$
	So we have
	\[
	\kappa(S_{L},R\setminus S_{R})\le|S_{L}|-|S_{R}|+\mu-n
	\]
	as desired.
\end{proof}


\subsubsection{Flow for Vertex Cuts}
\label{sec:flow_vertexcut}

The algorithm below is for finding sparse \emph{vertex cuts}. 


\global\long\def\vv{\mathsf{v}}
\global\long\def\vin{\mathrm{in}^{\vv}}
\global\long\def\vout{\mathrm{out}^{\vv}}


\SparseVertexCutLemma*
\begin{proof}
	For notational convenience, let us rename a graph that we want to
	find a vertex cut as $G^{\vv}=(V^{\vv},E^{\vv})$ where $A,B \subset V^\vv$. We use the standard
	reduction that splits each vertex into two vertices. More precisely,
	we construct a bipartite graph $G=(V=(L,R),E)$ as follows. For each
	vertex $v\in V^{\vv}$, we create $v_{L}\in L$ and $v_{R}\in R$
	and add a directed edge $(v_{L},v_{R})$ with capacity $\left\lfloor 1/\phi\right\rfloor $.
	For each each $(u,v)$, we add a directed edge $(u_{R},v_{L})$ with
	capacity $\infty$. For $v\in A$,
	we let $\Delta(v_{L})=1$. Set $\Delta(v)=0$ for all other vertices
	in $G$. For each $v\in B$, we let $T(v_{R})=1$. Set $T(v)=0$ for
	all other vertices in $G$. Let $c:E\rightarrow\mathbb{R}$ denote
	the edge capacity of edges in $G$. 
	
	Let $\Pi$ be the integral flow problem on $G$ defined by $(\Delta,T,c)$.
	We call \Cref{prop: preflow and label} with parameter $h=\frac{100\log(n/\phi)}{\phi}$ in $O(mh\log m)$
	and obtain a preflow $f$ in $G$. Set $z=\epsilon|A|$. There are
	two cases whether $\ex_{f}(V)\le z$ or not.
	
	If $\ex_{f}(V)\le z$, then by \Cref{rem:excess at source and path decomposition}, we can obtain a \emph{feasible} flow $\hat{f}$
	in $G$ with value at least $\Delta(V)-z=(1-\epsilon)|A|$. Moreover
	we can obtain a path decomposition $\pset_{\hat{f}}$ of $\hat{f}$
	in $O(\Delta(V)h)=O(nh)$ time. By reading the endpoint of paths in
	$\pset_{\hat{f}}$, we obtain an integral matching $M$ of size at
	least $(1-\epsilon)|A|$ from $A$ to $B$, such that $M$ can be
	embedded into $G^{\vv}$ with vertex congestion $\left\lfloor 1/\phi\right\rfloor $.
	This is because $\hat{f}$ corresponds to a flow in $G^{\vv}$ with
	vertex connection at most $\left\lfloor 1/\phi\right\rfloor $ by
	the construction of $G$. 
	
	If $\ex_{f}(V)>z$, then by \Cref{prop:excess give lower bound}, we
	know $|V_{h}|\ge\Delta(V_{h})>z$ and $|V_{0}|\ge T(V_{0})>z$ because
	$\forall v\in V,\Delta(v),T(v)\le1$. By \Cref{lem:bipartite label},
	$V_{h},V_{h-2},V_{h-4},\dots$ are subsets of $L$ and $V_{h-1},V_{h-3},V_{h-5},\dots$
	are subsets of $R$. Let $c'$ be an edge capacity function where $c_{0}(e)=c(e)$
	for all $e\in E(L,R)$ and $c_{0}(e)=0$ otherwise. Let $C=\sum_{e\in E}c_{0}(e)=n\left\lfloor 1/\phi\right\rfloor $.
	By the ball growing argument applying in two directions, there is
	an index $0\le i<h/2$ such that 
	$\vol^{c_{0}}(V_{h-2i}) \le\min\{\vol^{c_{0}}(V_{\ge h-2i}),\vol^{c_{0}}(V_{<h-2i})\}\cdot\frac{20\log C}{h}$.
	Otherwise, $\vol^{c_{0}}(V_{\ge h/2})\ge(1+\frac{20\log C}{h})^{h/2}>2C=\vol^{c_{0}}(V)$
	which is a contradiction. Fix such $i$ and let $S=V_{\ge h-2i}$. 
	Now, we bound the cut size of $S$:
	
	\begin{claim}\label{claim:bound vertex cut}
		$c(E(S,V\setminus S))\le\Delta(S)-T(S)+2\vol^{c_{0}}(V_{h-2i})$.
		In particular, $c(E(S,V\setminus S))$ is finite. 
	\end{claim}
	
	\begin{proof}
		First, observe that the total mass from $V_{h-2i-1}$ to $V_{h-2i}$
		is at most the total capacity of outgoing edges from $V_{h-2i}$ plus
		the sink capacity of of $V_{h-2i}$. That is, $f(V_{h-2i-1},V_{h-2i})\le c(E(V_{h-2i},V))+T(V_{h-2i-1})=c(E(V_{h-2i},V))$
		where $T(V_{h-2i})=0$ as $V_{h-2i}\subseteq L$. Now, we have the
		following: 
		\begin{align*}
		c(E(S,V\setminus S)) & =c(E(V_{h-2i},V_{h-2i-1}))+c(E(S,V\setminus S)\setminus E(V_{h-2i+1},V_{h-2i}))\\
		& \le c(E(V_{h-2i},V_{h-2i-1}))+\Delta(S)+f(V_{h-2i-1},V_{h-2i})-\ab_{f}(S)-\ex_{f}(S)\\
		& <\Delta(S)-T(S)-z+2c(E(V_{h-2i},V))\\
		& \le\Delta(S)-T(S)+2\vol^{c_{0}}(V_{h-2i})
		\end{align*}
		where the first inequality is by \Cref{prop:cap of skip}. The last
		inequality follows because $V_{h-2i}\subseteq L$ and so $c(E(V_{h-2i},V))=c(E(V_{h-2i},R))=c_{0}(E(V_{h-2i},R))=\vol^{c_{0}}(V_{h-2i})$.
	\end{proof}
	
	Let $(X,Y,Z,F)$ be a partition of vertices $V^{\vv}$ in $G^\vv$ defined as
	follow: If $v_{L},v_{R}\in S$, then $v\in X$. If $v_{L}\in S$ and
	$v_{R}\notin S$, then $v\in Y$. If $v_{L},v_{R}\notin S$, then
	$v\in Z$. If $v_{L}\notin S$ and $v_{R}\in S$, then $v\in F$. 
	\begin{claim}
		\label{claim:vertex neighbor}For any $U\subseteq V^{\vv}$, let $\vout(U)=\{v\notin U\mid\exists(u,v)\in E^{\vv}$
		where $u\in U\}$ and $\vin(U)=\{v\notin U\mid\exists(v,u)\in E^{\vv}$
		where $u\in U\}$ denote the set of out-neighbors and in-neighbors
		of $U$ respectively. We have $\vout(X)\subseteq Y$, $\vin(Z)\subseteq Y$,
		$\vout(F)\subseteq X\cup Y$, and $\vin(F)\subseteq Z\cup Y$. 
	\end{claim}
	
	\begin{proof}
		Otherwise, there exists an edge $e\in E(R\cap S,L\setminus S)$, which
		is impossible because $c(e)=\infty$ but $c(E(S,V\setminus S))$
		is finite.
	\end{proof}

	Now, we can define a vertex cut in $G^{\vv}$ that we will output. 
	Partition $F$ into two
	halves $F_{x},F_{z}$. 
	Our output is $(X\cup F_{x},Y,Z\cup F_{z})$.
	From \Cref{claim:vertex neighbor}, observe
	that $(X\cup F_{x},Y,Z\cup F_{z})$ is a vertex cut in $G^{\vv}$
	because $E^{\vv}(X\cup F_{x},Z\cup F_{z})=\emptyset$. 
	As both $|F_{x}|,|F_{z}|\ge|F|/3$, the following claim implies that
	$(X\cup F_{x},Y,Z\cup F_{z})$ is $O(\phi)$-vertex-sparse:
	
	\begin{claim}
		$|Y|\le O(\phi)\cdot\min\{|X\cup F|,|Z\cup F|\}$.
	\end{claim}
	
	\begin{proof}
		
		Recall that $\vol^{c_{0}}(V_{h-2i})\le\min\{\vol^{c_{0}}(V_{\ge h-2i}),\vol^{c_{0}}(V_{<h-2i})\}\cdot\frac{20\log C}{h}$
		by the choice of $i$. Now, observe that $\vol^{c_{0}}(V_{\ge h-2i})=\vol^{c_{0}}(S)=(2|X|+|Y|+ |F|)\cdot\left\lfloor 1/\phi\right\rfloor $,
		and $\vol^{c_{0}}(V_{<h-2i})=\vol^{c_{0}}(V\setminus S)=(2|Z|+|Y|+ |F|)\cdot\left\lfloor 1/\phi\right\rfloor $.
		Also, $c(E(S,V\setminus S))=|Y|\cdot\left\lfloor 1/\phi\right\rfloor $,
		$\Delta(S)=|X|+|Y|$ and $T(S)=|X|+|F|$. Recall that $h=\frac{100\log(n/\phi)}{\phi}$,
		so we have the following by \Cref{claim:bound vertex cut}:
		\begin{align*}
		|Y|\cdot\left\lfloor 1/\phi\right\rfloor  & \le(|X|+|Y|)-(|X|+|F|)+\min\{2|X|+|Y|+ |F|,2|Z|+|Y|+ |F|\}\cdot\left(2\cdot\left\lfloor 1/\phi\right\rfloor \cdot\frac{20\log(n/\phi)}{(\frac{100\log(n/\phi)}{\phi})}\right)\\
		& \le|Y|+\min\{|X|+|Y|+ |F|,|Z|+|Y|+ |F|\}.
		\end{align*}
		So $|Y|(\left\lfloor 1/\phi\right\rfloor  -2)\le\min\{|X\cup F|,|Z\cup F|\}$
		and so $|Y|\le O(\phi)\cdot\min\{|X\cup F|,|Z\cup F|\}$.		
	\end{proof}

	It remain so show that $(X\cup F_{x},Y,Z\cup F_{z})$ is $\Omega(\epsilon)$-vertex-balanced.
	Observe that $|X\cup Y\cup F|\ge|S|>z$ and $|Z\cup Y\cup F|\ge|V\setminus S|>z$.
	As we have $|Y|\le O(\phi)\cdot\min\{|X\cup F|,|Z\cup F|\}$, so $|X\cup F_{x}|,|Z\cup F_{z}|=\Omega(z)=\Omega(\epsilon n)$ by assuming that $\phi$ is smaller than a constant.
\end{proof}


\endinput


The input graph $G=(L,R,E)$ when we apply this algorithm will be obtained
by the standard reduction that splits each vertex $v$ into $v_{L}$
and $v_{R}$ and there is a directed edge $(v_{L},v_{R})$. So the
graph $G=(L,R,E)$ is bipartite and each vertex in $R$ has exactly
one in-degree. The algorithm either send a lot of flow or find a balanced
sparse cut. This sparse cut will correspond to a vertex sparse cut
in the original graph before splitting vertices.
\begin{lem}
[Global Flow for Vertex Cuts]\label{lem:global flow vertex cut}There
is a deterministic algorithm that, given a directed bipartite $m$-edge
graph $G=(V=(L,R),E)$ where each vertex $v\in R$ has in-degree at most
$1$, an excess parameter $z\ge0$, a height parameter $h\ge1$, and
a flow problem $\Pi=(\Delta,T,c)$ with total capacity from $L$ to
$R$ $C=\sum_{e\in E(L,R)}c(e)$, and the following holds
\begin{enumerate}
\item $\Delta(R)=0$, $T(L)=0$, $\Delta(L)\le T(R)$, 
\item $\forall v\in V,\Delta(v),T(v)\le1$, 
\end{enumerate}
in $O(mh\log m)$ time, either 
\begin{itemize}
\item returns a preflow $f$ with total excess $\ex_{f}(V)\le z$, or
\item returns a set $S\subset V$ where $|S|,|V\setminus S|>z$ and 
\[
c(E(S\cap L,\overline{S}\cap R))\le\Delta(S)-T(S)-z+\min\{\vol^{c'}(S),\vol^{c'}(V\setminus S)\}\cdot\frac{40\log C}{h}
\]
where $c'$ be an edge capacity function where $c'(e)=c(e)$ for all
$e\in E(L,R)$ and $c'(e)=0$ for all $e\notin E(L,R)$. 
\end{itemize}
\end{lem}

\begin{proof}
We call \Cref{prop: preflow and label} with parameter $h$ in $O(mh\log m)$.
Suppose that $\ex_{f}(V)>z$ otherwise we are done. By \Cref{prop:excess give lower bound},
we know $|V_{h}|\ge\Delta(V_{h})>z$ and $|V_{0}|\ge T(V_{0})>z$
because $\forall v\in V,\Delta(v),T(v)\le1$. By \Cref{lem:bipartite label},
$V_{h},V_{h-2},V_{h-4},\dots$ are subset of $L$ and $V_{h-1},V_{h-3},V_{h-5},\dots$
are subset of $R$. By the ball growing argument applying in two directions,
there is an index $0\le i<h/2$ such that $c'(E(V_{h-2i},V_{h-2i-1}))\le\min\{\vol^{c'}(V_{\ge h-2i}),\vol^{c'}(V_{<h-2i})\}\cdot\frac{20\log C}{h}$.
Otherwise, $\vol^{c'}(V_{\ge h/2})\ge(1+\frac{20\log C}{h})^{h/2}>2C$
which is a contradiction because $\vol^{c'}(V)=2\sum_{e\in E}c'(e)=2\sum_{e\in E(L,R)}c(e)=2C$.
Fix such $i$ and set $S=V_{\ge h-2i}$. As $S\supseteq V_{h}$ and
$S\cap V_{0}=\emptyset$ we have that $|S|,|V\setminus S|>z$. We
have, by \Cref{prop:cap of skip}, that 
\begin{align*}
c(E(S,V\setminus S)) & =c(E(V_{h-2i},V_{h-2i-1}))+c(E(V_{>h-2i},V_{\le h-2i})\setminus E(V_{h-2i+1},V_{h-2i}))\\
 & \le c'(E(V_{h-2i},V_{h-2i-1}))+\Delta(V_{\ge h-2i})+f(V_{h-2i-1},V_{h-2i})-\ab_{f}(V_{\ge h-2i})-\ex_{f}(V_{\ge h-2i})\\
 & <\Delta(S)-T(S)-z+2c'(E(V_{h-2i},V_{h-2i-1})).
\end{align*}
where the first inequality is because $V_{h-2i}\subset L$ and $V_{h-2i-1}\subset R$
and so $c(E(V_{h-2i},V_{h-2i-1}))=c'(E(V_{h-2i},V_{h-2i-1}))$, and
the second inequality follows by the $f(V_{h-2i-1},V_{h-2i})\le c'(E(V_{h-2i},V_{h-2i-1}))$.
Given this claim, we are done by the choice of $i$.

The claim follows because the total mass from $V_{h-2i-1}$ to $V_{h-2i}$
is at most the total capacity of incoming edges to $V_{h-2i-1}$ plus
the initial mass at $V_{h-2i-1}$. Note that $V_{h-2i-1}\subseteq R$,
so $\Delta(V_{h-2i-1})=0$. That is, $f(V_{h-2i-1},V_{h-2i})\le c(L\cup R,V_{h-2i-1})+\Delta(V_{h-2i-1})$.
As $V_{h-2i-1}\subseteq R$, so $\Delta(V_{h-2i-1})=0$. As every
vertex in $R$ has exactly one in-degree, and each vertex in $V_{h-2i-1}$
has one in-degree from $V_{h-2i}$, so $c(L\cup R,V_{h-2i-1})\le c(V_{h-2i},V_{h-2i-1})$.
Therefore, we have $f(V_{h-2i-1},V_{h-2i})\le c(E(V_{h-2i},V_{h-2i-1}))=c'(E(V_{h-2i},V_{h-2i-1}))$.
\end{proof}
\SparseVertexCutLemma*


==> more_analysis.tex <==

\section{More Applications of Adaptive Flow Analysis}

\label{sec:more analysis}
\begin{thm}
There is a deterministic algorithm that, given a decremental bipartite
graph $G$ with $m$ edges, maintain a $(1+\epsilon)$-approximate
fractional matching of $G$ in $\tilde{O}(m)$ time.
\end{thm}

\begin{thm}
There is a deterministic algorithm that, given a decremental graph
$G$ with $n$ vertices and $m$ edges and $s,t\in V(G)$, maintain
a $(1+\epsilon)$-approximate $s$-$t$ vertex max flow of $G$ in
$\tilde{O}(mn)$ time.
\end{thm}



